Generating Educational Materials with Different Levels of Readability using LLMs

This study introduces the leveled-text generation task, aiming to rewrite educational materials to specific readability levels while preserving meaning. We assess the capability of GPT-3.5, LLaMA-2 70B, and Mixtral 8x7B, to generate content at various readability levels through zero-shot and few-shot prompting. Evaluating 100 processed educational materials reveals that few-shot prompting significantly improves performance in readability manipulation and information preservation. LLaMA-2 70B performs better in achieving the desired difficulty range, while GPT-3.5 maintains original meaning. However, manual inspection highlights concerns such as misinformation introduction and inconsistent edit distribution. These findings emphasize the need for further research to ensure the quality of generated educational content.

==> sections/content.tex <==
% - We are working on this particular task called ``Leveled Text Generation'', where given a source text, we would like to rewrite that text within a certain difficult level. (This task is particular important for education purpose)
% - At the moment, using a dataset, we found that, basically all the model performs poorly and in different ways.
% - In creative writing context, people often argue that all the generated texts are somewhat useful for writers as they might inspire writers in different ways or different time (like inception).
% - However, in this particular task, we need precise information and we do not expect the text to be deviated from the original text too much (in the semantic space).
% - Obviously, the current LLMs can not do this. (yeah but we did not try GPT-4 because it is expensive)

% - Given all these constraints, we believe that this work should be solve in the HCI domain, where an interface/system is needed to help people (1) quickly traverse the generated texts, (2) make decisions on what to use and what to reject, (3) provide a avaliability to write when all the suggestions are really bad, (4) combine the strength from multiple models/single models' different outputs.

% Future: we can also learn a model to automatically generate (select) a text based on multiple generated texts.

% How to do:
% - overgeneration from one or multiple models
% - alignment
% - interface


\section{Introduction}
Adapting educational content to suit diverse learning needs is crucial yet complex.
The task, referred as ``Leveled Text Generation,'' involves adjusting the difficulty of texts (either easier or harder to read) without losing their original meaning.
Content curators often struggle to write texts within a desired difficulty range, and thus a time-consuming back-and-forth process is always needed when curating such contents.
LLMs, in particular the chat interface of the ChatGPT, do not eliminate the back-and-forth process due to the poor performance in reaching the desired difficulty level.
%
Although the unpredictability of machine-generated texts can be helpful in creative writing, offering fresh perspectives and ideas,
this variability is less desirable for the leveled text generation task.
Here, the goal is to convey the same information accurately at an adjusted difficulty level.

\input{table/llm-performance}

\Cref{tab:llm-performance} shows the performance of different LLMs.
The extremely low Match score indicates that models, in general, can not reach to the target difficult level within one single try no mater what technique is used.
The Direction score suggests that best-performing models can at least move toward the right direction per request at around 80\% success rate.
The BERTScore, on the other hand, shows that most of the model can preserve the meaning of the texts when rewriting.

\section{A Human-Centered Solution}
Given the fact that current LLMs can not effectively solve the task, we believe the leveled text generation task should be tackled as an HCI task.
Here are a set of considerations:
\begin{itemize}
    \item
    \textbf{Quickly Browse}: Users can easily navigate through many generated text options.

    \item
    \textbf{Make Informed Choices}: The system helps users identify and select the most suitable texts that meet the criteria.

    \item
    \textbf{Merge the Best Elements}: The system should combine or help users combine the best parts of multiple texts generated by one or multiple models.

    \item
    \textbf{Edit When Needed}: Users can directly edit or write new content if the generated responses do not meet their needs.
    
\end{itemize}

\subsection{Proposed Solution}
The overall workflow includes an offline pre-processing stage and a user interface (actual system).
\begin{itemize}
    \item
    \textbf{Over-generation (pre-processing)}: Generate responses multiple times from multiple models to create a response bank that include variety of signature of texts.

    \item 
    \textbf{Alignment (pre-processing)}: Most of the editing would be done in sentence-level to word-level. As a result, alignments between all the responses should be obtained for processing.

    \item
    \textbf{Analyzing Lexile Scores (pre-processing)}: Analyze the difficulty level for each of the responses. Such information will be used for selecting responses in the user-facing system.

    \item
    \textbf{User interface}. A text editor that can provide feedback instantly (with minimum response time) to help users navigate through all the possible texts: (1) Auto-complete; (2) drag-and-drop; etc.
\end{itemize}


\section{Expected Results}
...

